Guarded Variable Automata over Infinite Alphabets

We define guarded variable automata (GVAs), a simple extension of finite automata over infinite alphabets. In this model the transitions are labelled by letters or variables ranging over an infinite alphabet and guarded by conjunction of equalities and disequalities. GVAs are well-suited for modeling component-based applications such as web services. They are closed under intersection, union, concatenation and Kleene operator, and their nonemptiness problem is PSPACE-complete. We show that the simulation preorder of GVAs is decidable. Our proof relies on the characterization of the simulation by means of games and strategies. This result can be applied to service composition synthesis.

==> epsilonFVA.tex <==
The class of GVAs with $\eps$-transitions will be denoted by $\eps$-GVAs. 
We emphasize that the $\eps$-transitions are not guarded.   
\begin{myclaim}
\label{eps:closed:lemma}
For a $\eps$-GVA $\mycal{A}^{\eps}$  there exists a GVA $\mycal{A}$ (without $\eps$-transitions)
satisfying $L(\mycal{A})=L(\mycal{A}^{\eps})$.
\end{myclaim}
\begin{proof}
The construction of a GVA  out of a $\eps$-GVA 
 is more subtle than the  construction known for FAs 
 since we need to take into account the refreshing of the variables.
We define an operator $\Theta$ that transforms  a $\eps$-GVA  
to an  equivalent $\eps$-GVA with strictly less $\eps$-transitions. Thus the desired 
    GVA without $\eps$-transitions is the least fixed-point of $\Theta$.
Intuitively, the operator $\Theta$ eliminates all the $\eps$-transitions 
which are preceded by a non $\eps$-transition.   

%$\mycal{A}$ as an extension of $\mycal{A}^{\eps}$ as follows.
  Assume $\mycal{A}^{\eps}=\model{\Sigma,\mycal{X},Q^{\eps},Q_0^{\eps},F^{\eps},\delta^{\eps},\kappa^{\eps}}$.
Let $\Upsilon(q)$ be the set of states that are reachable from state $q$ by following an $\eps$-transition
 and let $\Upsilon(Q')=\set{\Upsilon(q)| q \in Q'}$, for  $Q' \subseteq Q^\eps$. 
  Let
  $\Theta(\mycal{A}^{\eps})=\model{\Sigma,\mycal{X},Q,Q_0,F,\delta,\kappa}$
  where:
  \begin{align*}
    Q  &= Q^\eps \cup (Q^\eps \times Q^\eps) \\
    & \pi_1:\mycal{P}(Q) \to \mycal{P}(Q^\eps)\\
    & \quad \quad Q' \mapsto \set{ p \,\vert\, (p,q)\in Q'} \\    
    & \pi_2: \mycal{P}(Q) \to \mycal{P}(Q^\eps)\\
    & \quad \quad Q' \mapsto \set{ q \,\vert\, (p,q)\in Q'} \\    
    Q_0 &=Q_0^\eps \cup \Upsilon(Q_0^\eps) \cup \pi_1^{-1}(Q_0^\eps) \\
    F &=F^\eps \cup \Upsilon^{-1}(F^\eps) \cup \pi_2^{-1}(F^\eps)\\
    \delta&= \set{p\uberTo{\alpha,g}q \in \delta^\eps \gvert \alpha \neq \eps } \cup  
    \set{q_1\uberTo{\alpha,g}(q_2,q_3) \gvert q_1\uberTo{\alpha,g}q_2\uberTo{\eps} q_3 \in \delta^\eps \gvert \alpha \neq \eps} \cup \\
        & \quad \;    \set{(q_1,q_2)\uberTo{\alpha,g}q_3 \gvert q_2\uberTo{\alpha,g} q_3 \in \delta^\eps }
       \cup \set{q_1 \uberTo{\eps} q_2 \gvert {\nexists} q_0\uberTo{\alpha,g} q_1 \tst \alpha \neq \eps}\\
     \kappa&=\kappa^{\eps} \cup (\pi_1^{-1} \circ \kappa^\eps) \cup (\pi_2^{-1} \circ \kappa^\eps)
  \end{align*}
%The intuition behind  a state $(p,q)$ of $\Theta(\mycal{A}^{\eps})$ is that it corresponds to the state $q$ of 
% $\mycal{A}^\eps$ reached by a transition from $p$.   
%The construction of $Q$ out of $Q^{\eps}$ allows us to define a  function  
%$\psi: Q \uberTo{} Q^\eps$ as $\psi(q)=q$ if $q \in Q^{\eps}$ and $\psi((q_1,q_2))=q_1$.



In order to prove that $L(\Theta(\mycal{A}^{\eps}))=L(\mycal{A}^{\eps})$, it suffices to prove 
 the following three Claims, the first one is straightforward:

\begin{trivlist}
  \item \textbf{Fact 1.} \it Every accepting run in $\mycal{A}^{\eps}$
    that does not follow any $\eps$-transition is still an accepting run  
    in $\Theta(\mycal{A}^{\eps})$. Conversely,  every accepting run in $\Theta(\mycal{A}^{\eps})$
    that passes only through states in $Q^{\eps}$ is still an accepting run in $\mycal{A}^\eps$.
\end{trivlist}

  \begin{trivlist}
  \item \textbf{Fact 2.} \it There exists a run 
    \begin{align*}
      q_0,M_0   \uberTo{\alpha,g} q_1,M_1  \uberTo{\eps} q_{2},M_{2} 
    \end{align*}
  in $\mycal{A}^{\eps}$ with $\alpha \neq \eps$ 
    \emph{iff}  there exists a run
    \begin{align*}
      q_0,M_0 \uberTo{\alpha,g}  (q_1,q_2),M'_2
    \end{align*}
in $\Theta(\mycal{A}^{\eps})$ such that  $M_2=M'_2$.

  \end{trivlist}
  \begin{trivlist}
  \item \textbf{Proof of the Fact 2.}
    \begin{itemize}
    \item[$\Rightarrow$)] From the definition of $Q$ and $\delta$ it follows that 
      $(q_0,q_1) \in \delta(q_0,\alpha)$, and it remains to show that $M_2=M'_2$. 
      We only discuss the case when $\alpha$ is a letter in $\Sigma$, the case when it 
      is a variable can be handled similarly. 
      On the one hand, $M_2={M_1}_{|D_2}$ where $D_2=Dom(M_1) \setminus  (\kappa^{\eps})^{-1}(q_2)$, 
      and $M_1=(M_0 \uplus \gamma)_{|D_1}$ where $D_1=Dom(M_0) \setminus  \kappa^{-1}(q_1)$ and $\gamma$ is a substitution 
      such  that $\gamma \models M_0(g)$. Hence
      $M_2={M_0}_{|D}$ where  $D=(Dom(M_0) \uplus dom(\gamma)) \setminus  \big((\kappa^{\eps})^{-1}(q_1) \cup (\kappa^{\eps})^{-1}(q_2)\big)$.
On the other hand, we have $M'_2=(M_0 \uplus dom(\gamma)) \setminus D'$, where $D'=Dom(M_0) \setminus  \kappa^{-1}((q_1,q_2))$.
  It follows from the definition of $\kappa$, the refreshing function 
   of $\Theta(\mycal{A}^{\eps})$, that $\kappa^{-1}((q_1,q_2))=(\kappa^{\eps})^{-1}(q_1) \cup (\kappa^{\eps})^{-1}(q_2)$.
   Hence, $D=D'$ and $M_2=M'_2$.

    \item[$\Leftarrow$)] This direction is proved by following the same reasoning made in   the direction $(\Rightarrow)$
   on the      refreshing  function. 
 \end{itemize} 
This ends the proof of Fact 2. \qed
%

  \begin{trivlist}
  \item \textbf{Fact 3.} \it Let $q_1  \in Q^{\eps}$  and $(q_0,q_1) \in Q$. There exists a run 
    \begin{align*}
      q_1,M_1   \uberTo{\alpha,g} q_2,M_2 
    \end{align*}
  in $\mycal{A}^{\eps}$ %with $\alpha \neq \eps$ 
    \emph{iff}  there exists a run
    \begin{align*}
      (q_0,q_1),M_1 \uberTo{\alpha,g}  q_2,M_2
    \end{align*}
in $\Theta(\mycal{A}^{\eps})$.
  \end{trivlist}
 \begin{trivlist}
  \item \textbf{Proof of Fact 3.}
 By checking the transition function $\delta$. \qed
  \end{trivlist}
%
To accomplish the proof, it remains to notice that 
 if $q \in Q$ is such that $q \notin \pi_{1}^{-1}(Q^{\eps})$, then 
 the outgoing transitions  from $q$ in $\mycal{A}^{\eps}$  are exactly 
  the outgoing transitions from $q$ in $\Theta(\mycal{A}^{\eps})$.
\end{trivlist}
\qed
\end{proof}
 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 


==> flight.tex <==
\section{Motivating example: flight reservation}
Figure \ref{flight:example:fig} depicts a service composition problem of a Flight Reservation Web site allowing 
clients to authenticate, book flights and pay. Clients are interacting with three services 
\ttt{\uppercase{Authentification}},  
\ttt{\uppercase{Flight}} and \ttt{\uppercase{Payment}}.
The Authentification service requires the variables \ttt{Id} 
(identifier)  and \ttt{Pwd}  (password) of the client to allow him to log in.
The payment service requires the variables \ttt{Owner}, \ttt{Nbr}, \ttt{CSC} and \ttt{Exp} 
for respectively card holder, card number, card security code and expiration date. 
It works under some guards where it generates the cryptogram of the card number, 
the expiration date and 
the security code  with a key \ttt{K} and checks wether it is to equal \ttt{CSC}. 
In this case  the payment is done sucessfully. Otherwise, it is rejected.
The Flight service requires the  variables \ttt{From}, \ttt{To}, \ttt{Dpt} and \ttt{Ret} 
for the following information: flying from, flying to, departing time and returning time.
It sends the client the number of his ticket (\ttt{Tck}$\_$\ttt{Nr}) once the flight is booked. 

\begin{figure}[tbh*]
  \vspace{-10pt}
\begin{center}
\scalebox{0.7}{\begin{tikzpicture}[shorten >=1pt,node distance=1.8cm, bend angle=60,
   on grid,auto, initial text=, >=stealth] 
   \node[state,initial] (p_0)   {$p_0$}; 
   \node[state](p_1) [below =of p_0] {$p_1$}; 
   \node[state](p_2) [below =of p_1] {$p_2$};
   \node[state](p_3) [below =of p_2] {$p_3$};
   \node[state](p_4) [below =of p_3] {$p_4$};
	\node[state](p_5) [below =of p_4] {$p_5$};
	\node[state](p_6) [below =of p_5] {$p_6$};
	\node[state](p_7) [below =of p_6] {$p_7$};
	\node[state](p_8) [below =of p_7] {$p_8$};
%	\node[state](p_9) [below =of p_8] {$p_9$};
%	\node[state](p_10) [below =of p_9] {$p_{10}$};
%   \node[state](p_11) [below =of p_10] {$p_{11}$};
    \path[->] 
    %%--------- Interaction with AUTHENTIFICATION Service---------------
    (p_0) edge   node  [left] {\ttt{f(Id,Pwd)}}(p_1)
    (p_1) edge   node  [left] {\ttt{f(Id,Ok$\_$auth)}} (p_2)
	 (p_1) edge  [bend right] node [right] {\ttt{f(Id,Err$\_$auth)}}  (p_0)
     %%------------------------------------------------------------------
    %%--------- Interaction with FLIGHT Service--------------------

    (p_2) edge   node  [left] {\ttt{f(Id,From,To,Dpt,Ret,Req$\_$Conf)}} (p_3)
    (p_3) edge  [bend right] node [right]  {\ttt{f(Id,Err$\_$Rv)}} (p_2)
    %%--------- Interaction with Payment Service--------------------
    (p_3) edge   node  [left] {\ttt{f(Id,Req$\_$Pay)}}(p_4)
    (p_4) edge   node  [left] {\ttt{f(Id,Owner,Nbr,CSC,Exp)}}(p_5)
    (p_5) edge   node  [left] {\ttt{f(Id,Ok$\_$Pay)}}(p_6)

    (p_5) edge    [bend right] node [right] {\ttt{f(Id,Err$\_$Pay)}}(p_3)
%    (p_6) edge   node  [left] {\ttt{(C$_{i}$,?Thks$\_$Pay))}}(p_7)
    (p_6) edge   node  [left] {\ttt{f(Id,Proof$\_$Pay)}}(p_7)
    (p_7) edge   node  [left] {\ttt{f(Id,Tck$\_$Nr)}}(p_8)
    (p_8) edge  [bend left,out=90,in=100] node [left]  {\ttt{f(Id,Quit)}} (p_2)
    (p_2) edge  [bend left] node [left]  {\ttt{f(Id,log$\_${out})}} (p_0)
    %%------------------------------------------------------------------
    -- (0,0.8) node {CLIENT};
    %%------------------------------------------------------------------

% ------------   Service Authentification   -----------------
  \begin{scope}[xshift=8cm, yshift=0cm,node distance=1.8cm]
   \node[state,initial] (q_0)   {$q_0$}; 
   \node[state] (q_1) [below =of q_0] {$q_1$}; 
   \node[state] (q_2) [below =of q_1] {$q_2$}; 
    \path[->] 
    (q_0) edge   node [left] { \ttt{f(Id,Pwd)}} (q_1)
    (q_1) edge  [bend right] node [right] {\ttt{f(Id,Err$\_$auth)}} (q_0)
    (q_1) edge   node [right] {\ttt{f(Id,OK$\_$auth)}} (q_2)
	 (q_2) edge  [bend left] node [left]  {\ttt{f(Id,log$\_${out})}} (q_0)
    -- (0,0.8) node {AUTHENTIFICATION};
  \end{scope}
%-------------------------------------------------------------

% ------------   Service FLIGHT   -----------------
  \begin{scope}[xshift=8cm, yshift=-6 cm,node distance=1.8cm]
   \node[state,initial] (r_0)   {$r_0$}; 
   \node[state] (r_1) [below =of r_0] {$r_1$}; 
   \node[state] (r_2) [below =of r_1] {$r_2$}; 
   \node[state] (r_3) [below =of r_2] {$r_3$}; 
%   \node[state] (r_4) [below =of r_3] {$r_4$}; 
%   \node[state] (r_5) [below =of r_4] {$r_5$}; 
    \path[->] 
    (r_0) edge  node [left] {\ttt{f(Id,From,To,Dpt,Ret,Req\_Conf)}}(r_1)
	 (r_1) edge [bend right,out=-90,in=-100] node [right] {\texttt{f(Id,Err$\_$Rv)}} (r_0)
    (r_1) edge  node [left] { \ttt{f(Id,Proof$\_$Pay)}} (r_2)
    (r_2) edge  node [left] { \ttt{f(Id,Tck$\_$Nr)}} (r_3)
    (r_3) edge [bend right,out=-90,in=-90] node [right] {\ttt{f(Id,Quit)}} (r_0)
    -- (0,0.8) node {FLIGHT};
  \end{scope}
%-------------------------------------------------------------

% ------------   Service Payment   -----------------
  \begin{scope}[xshift=8cm, yshift=-13.8cm,node distance=1.8cm]
   \node[state,initial] (t_0)   {$t_0$}; 
   \node[state] (t_1) [below =of t_0] {$t_1$}; 
   \node[state] (t_2) [below =of t_1] {$t_2$}; 
%   \node[state] (t_3) [below =of t_2] {$t_3$}; 
    \path[->] 
    (t_0) edge  node [left] { \ttt{f(Id,Req$\_$Pay)}} (t_1)
    (t_1) edge  node [left] {\ttt{f(Id,Owner,Nbr,CSC,Exp)}}(t_2)


%    (t_2) edge  [bend right] node [right] { \ttt{(SP,!f(Id,Ok$\_$Pay)) if CSC = Crypt$_{K}$(Nbr,CSC,Exp)}} (t_0) 

(t_2) edge  [bend right] node [right] {\shortstack[l] {\ttt{f(Id,Ok$\_$Pay),} \\ \ttt{CSC = Crypt$_{K}$(Nbr,CSC,Exp)}} }(t_0) 

%\shortstack[l]{texte sur\\
%   plusieurs lignes}

    (t_2) edge  [bend left] node [left] {\ttt{f(Id,Err$\_$Pay)}} (t_0)
%    (t_3) edge [bend right,out=-90,in=-90] node [right] { \ttt{(SP,!Thks$\_$Pay)}} (t_0)
    -- (0,0.8) node {PAYMENT};
  \end{scope}
%-------------------------------------------------------------
\end{tikzpicture}}
\end{center}
  \vspace{-22pt}
\caption{Flight reservation example}
  \vspace{-10pt}
\label{flight:example:fig}
\end{figure}

